ScaleEdit-12M: Scaling Open-Source Image Editing Data Generation via Multi-Agent Framework

Instruction-based image editing has emerged as a key capability for unified multimodal models (UMMs), yet constructing large-scale, diverse, and high-quality editing datasets without costly proprietary APIs remains challenging. Previous image editing datasets either rely on closed-source models for annotation, which prevents cost-effective scaling, or employ fixed synthetic editing pipelines, which suffer from limited quality and generalizability. To address these challenges, we propose ScaleEditor, a fully open-source hierarchical multi-agent framework for end-to-end construction of large-scale, high-quality image editing datasets. Our pipeline consists of three key components: source image expansion with world-knowledge infusion, adaptive multi-agent editing instruction-image synthesis, and a task-aware data quality verification mechanism. Using ScaleEditor, we curate ScaleEdit-12M, the largest open-source image editing dataset to date, spanning 23 task families across diverse real and synthetic domains. Fine-tuning UniWorld-V1 and Bagel on ScaleEdit yields consistent gains, improving performance by up to 10.4% on ImgEdit and 35.1% on GEdit for general editing benchmarks and by up to 150.0% on RISE and 26.5% on KRIS-Bench for knowledge-infused benchmarks. These results demonstrate that open-source, agentic pipelines can approach commercial-grade data quality while retaining cost-effectiveness and scalability. Both the framework and dataset will be open-sourced.

==> preamble.tex <==
\definecolor{citecolor}{HTML}{0071BC}

\definecolor{oursgray}{gray}{0.93} 


% define new commands here
\newcommand{\modelname}{InternVL-U\xspace}

%%%%%%%%%%%%
% Add a period to the end of an abbreviation unless there's one
% already, then \xspace.
\RequirePackage{xspace}
\makeatletter

\DeclareRobustCommand\onedot{\futurelet\@let@token\@onedot}
\def\@onedot{\ifx\@let@token.\else.\null\fi\xspace}

\def\eg{\textit{e.g}\onedot} 
\def\Eg{\textit{E.g}\onedot}
\def\ie{\textit{i.e}\onedot} 
\def\Ie{\textit{I.e}\onedot}
\def\cf{\emph{cf}\onedot} 
\def\Cf{\emph{Cf}\onedot}
\def\etc{\emph{etc}\onedot} 
\def\vs{\emph{vs}\onedot}
\def\wrt{w.r.t\onedot} 
\def\dof{d.o.f\onedot}
\def\iid{i.i.d\onedot} 
\def\wolog{w.l.o.g\onedot}
\def\etal{\emph{et al}\onedot}

\makeatother

%%%%%%%%%%%%

\newcommand{\yes}{\ding{51}}
\newcommand{\no}{\ding{55}}
\newcommand{\graybox}[1]{\colorbox{gray!15}{#1}}
\newcommand{\gbf}[1]{\green{\bf{\fn{(#1)}}}}
\newcommand{\rbf}[1]{\gray{\bf{\fn{(#1)}}}}
\newcommand{\lsp}{\ \ \ \ --\ ~}
\newcommand{\rsp}{\ \ --\ \ \ ~}

\usepackage{CJK}


\newcommand{\TODO}[1]{\begin{CJK}{UTF8}{gbsn}\textcolor{red}{[todo: #1]}\end{CJK}}

\newcommand{\prompt}[1]{\textcolor{black}{\footnotesize{\texttt{#1}}}}


% \definecolor{myblue}{HTML}{3859FF}
% \definecolor{myblue}{HTML}{DEF2FA}
\definecolor{myblue}{HTML}{d6f0ff}
% \definecolor{myblue}{HTML}{DBF5F0}
% \definecolor{myblue}{HTML}{C0DEFA}

\newcommand{\mytoprule}{
    \toprule
    \noalign{\vspace{-0.2mm}}
}

\newcommand{\mymidrule}{
    \noalign{\vspace{-0.8mm}}
    \midrule
    \noalign{\vspace{-1mm}}
}

\newcommand{\mybottomrule}{
    \noalign{\vspace{-0.6mm}}
    \bottomrule
}

\hyphenation{InternVL}

% table
\newcommand{\tablestyle}[2]{\setlength{\tabcolsep}{#1}\renewcommand{\arraystretch}{#2}\centering\footnotesize}

% \newcommand\blfootnote[1]{%
% \begingroup
% \renewcommand\thefootnote{}\footnote{#1}%
% \addtocounter{footnote}{-1}%
% \endgroup
% }

\definecolor{baselinecolor}{gray}{.9}
\definecolor{reduce-color}{RGB}{67,178,68}
\newcommand{\gray}[1]{\textcolor{gray}{#1}}
\newcommand{\green}[1]{\textcolor[RGB]{96,177,87}{#1}}
\newcommand{\fn}[1]{\footnotesize{#1}}

% 定义自己的颜色
\definecolor{lightblue}{RGB}{152,182,234}
\definecolor{lightgreen}{RGB}{164,212,133}

\definecolor{cvprblue}{rgb}{0.21,0.49,0.74}
\definecolor{prompt}{rgb}{0.21,0.49,0.74}

\usepackage{array}

\usepackage[most]{tcolorbox}
\newcommand{\finding}[2]{
    % args:
    %   1: finding number
    %   2: finding text
    \vspace{-0.1cm}
    \begin{tcolorbox}[
        colback=white!90!gray,     % Soft ivory background
        colframe=teal!60!black,     % Deep navy frame color
        arc=5pt,                    % Less rounded corners for a modern look
        boxsep=5pt,                 % Inner margin between text and frame
        left=6pt,                  % Left margin within the box
        right=6pt,                 % Right margin within the box
        top=2pt,                    % Top margin within the box
        bottom=2pt,                 % Bottom margin within the box
        boxrule=0.8pt,              % Frame thickness
        drop shadow=gray!50!white,  % Subtle shadow effect for depth
        enhanced jigsaw             % Allows for the shadow effect and better arcs
    ]
    \vspace{-0.1cm}
        \paragraph{\textbf{\textit{Observation #1:}}}#2
    \vspace{-0.1cm}
    \end{tcolorbox}
    \vspace{-0.1cm}
}

\usepackage{textcomp}

% 自动开启和关闭中文环境
%%
\AtBeginDocument{\begin{CJK}{UTF8}{gbsn}\CJKtilde}
\AtEndDocument{\clearpage\end{CJK}}
%%

\definecolor{BoxBackground}{RGB}{240, 240, 240} % 浅灰色背景
\definecolor{BoxFrame}{RGB}{0, 0, 0} % 黑色边框
\definecolor{TitleBackground}{RGB}{0, 0, 0} % 标题背景颜色
\definecolor{TitleText}{RGB}{255, 255, 255} % 标题文字颜色
% 设置全局tcolorbox样式
\tcbset{
  academicbox/.style={
    boxsep=5pt,
    left=2pt,
    right=2pt,
    bottom=0.5pt,
    boxrule=0.5pt,
    colback=BoxBackground,
    colframe=BoxFrame,
    colbacktitle=TitleBackground,
    coltitle=TitleText,
    enhanced,
    attach boxed title to top left={yshift=-0.1in,xshift=0.1in},
    boxed title style={boxrule=0pt,colframe=white},
    title={#1},
  }
}
\newtcolorbox{AcademicBox}[1][]{academicbox=#1}
\newcommand{\nchar}{\textbackslash n}
